AIGVE-Tool: AI-Generated Video Evaluation Toolkit with Multifaceted Benchmark

The rapid advancement in AI-generated video synthesis has led to a growth demand for standardized and effective evaluation metrics. Existing metrics lack a unified framework for systematically categorizing methodologies, limiting a holistic understanding of the evaluation landscape. Additionally, fragmented implementations and the absence of standardized interfaces lead to redundant processing overhead. Furthermore, many prior approaches are constrained by dataset-specific dependencies, limiting their applicability across diverse video domains. To address these challenges, we introduce AIGVE-Tool (AI-Generated Video Evaluation Toolkit), a unified framework that provides a structured and extensible evaluation pipeline for a comprehensive AI-generated video evaluation. Organized within a novel five-category taxonomy, AIGVE-Tool integrates multiple evaluation methodologies while allowing flexible customization through a modular configuration system. Additionally, we propose AIGVE-Bench, a large-scale benchmark dataset created with five SOTA video generation models based on hand-crafted instructions and prompts. This dataset systematically evaluates various video generation models across nine critical quality dimensions. Extensive experiments demonstrate the effectiveness of AIGVE-Tool in providing standardized and reliable evaluation results, highlighting specific strengths and limitations of current models and facilitating the advancements of next-generation AI-generated video techniques.

==> tables/auto_corr.tex <==
\begin{table*}[h]
    \centering
    \small
    \scalebox{0.70}{

    \begin{tabular}{l|ccccccccc}
        \toprule
        Videoscore & Technical\_Quality & Dynamic & Consistency & Physics & Element\_Pre & Element\_Qu & Element\_Act\_Pre & Element\_Act\_Qu & Overall \\
        \midrule
        dynamic\_deg & -0.159/-0.12/-0.227 & -0.082/-0.065/-0.1 & -0.129/-0.101/-0.18 & 0.056/0.044/0.053 & 0.052/0.042/0.026 & -5.7503 & 0.048/0.039/0.008 & -16.4706 & -0.091/-0.067/-0.144 \\
        factual\_cons & -0.164/-0.122/-0.205 & -0.14/-0.112/-0.125 & -0.057/-0.043/-0.118 & 0.194/0.157/0.168 & 0.023/0.018/-0.033 & -8.0808 & -0.117/-0.089/-0.146 & -42.2535 & -0.173/-0.128/-0.194 \\
        temporal\_co & -0.119/-0.088/-0.175 & -0.118/-0.094/-0.098 & -0.002/0.001/-0.083 & 0.212/0.171/0.165 & 0.044/0.036/-0.010 & -9.9206 & -0.092/-0.071/-0.121 & 0.014/0.013/-0.055 & -0.131/-0.097/-0.16 \\
        text\_to\_vide & -0.095/-0.069/-0.18 & -0.101/-0.081/-0.085 & -0.026/-0.019/-0.093 & 0.201/0.162/0.168 & 0.097/0.077/0.042 & -8.4280 & -0.031/-0.024/-0.054 & 0.015/0.016/-0.053 & -0.073/-0.051/-0.116 \\
        \midrule
        videophy & 0.001/-0.000/0.032 & 0.040/0.031/0.035 & -424.2424 & -31.0421 & 0.008/0.007/0.029 & -0.013/-0.01/0.005 & 0.119/0.091/0.108 & 0.027/0.020/0.061 & 0.097/0.070/0.097 \\
        \bottomrule
    \end{tabular}

    
    }
    
    \caption{Comparison of different video scores across various evaluation metrics.}
    \label{tab:videoscore}
\end{table*}

==> tables/instructions_description.tex <==
\begin{table}[ht]
    \centering
    \small % Reduces font size
    \renewcommand{\arraystretch}{1.0} % Adjusts row height for compactness
    \setlength{\tabcolsep}{4pt} % Reduces column spacing
    \scalebox{0.75}{
    \begin{tabular}{l|c c}
        \toprule
        \textbf{Category} & \textbf{Objects} & \textbf{Dynamic} \\
        \midrule
        \textbf{\textit{Global View}} & 
        \begin{tabular}[c]{@{}l@{}}
            Mountains, Oceans, Plains, \\ 
            Rivers, Lakes, Deserts, Cities, \\ 
            Architecture, Streets 
        \end{tabular} & 
        \begin{tabular}[c]{@{}l@{}}
            Camera Movements, Daylight \\ 
            Transitions, Weather Changes, \\ 
            Seasonal Shifts 
        \end{tabular} \\
        \midrule
        \textbf{\textit{Close Shot}} & 
        \begin{tabular}[c]{@{}l@{}}
            Humans, Animals, Plants, Objects 
        \end{tabular} & 
        \begin{tabular}[c]{@{}l@{}}
            Single-Object Actions, \\ 
            Multiple-Object Interactions 
        \end{tabular} \\
        \bottomrule
    \end{tabular}    
    }
    \caption{Summary of Instruction Categories}
    \label{tab:instructions_description}
\end{table}


==> tables/video_specs.tex <==
\begin{table}[!t]
    \centering
    \small
    \begin{tabular}{l|r r r}
        \toprule
        \textbf{Model} & \textbf{Resolution} & \textbf{Frame Rate} & \textbf{Duration} \\
        \midrule
        \textbf{CogVideoX} \cite{yang2024cogvideox} & 1360 $\times$ 768 & 16 fps & 5s \\
        \textbf{Genmo} \cite{genmo2024mochi} & 848 $\times$ 480 & 30 fps & 5s \\
        \textbf{Hunyuan} \cite{kong2025hunyuanvideosystematicframeworklarge} & 960 $\times$ 544 & 24 fps & 5s \\
        \textbf{Pyramid} \cite{jin2024pyramidal} & 1280 $\times$ 768 & 24 fps & 5s \\
        \textbf{Sora} \cite{sora2024} & 854 $\times$ 480 & 30 fps & 5s \\
        \bottomrule
    \end{tabular}
    \caption{Specifications of Generated Videos from each Model.}
     \label{tab:video_specs}
\end{table}

